The partition algebra and the plethysm coefficients I: stability and Foulkes' conjecture

We propose a new approach to study plethysm coefficients by using the Schur-Weyl duality between the symmetric group and the partition algebra. This allows us to explain the stability properties of plethysm and Kronecker coefficients in a simple and uniform fashion for the first time. We prove the strengthened Foulkes' conjecture for stable plethysm coefficients in an elementary fashion.

==> hobby.code.tex <==
%%
%% This is file `hobby.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% hobby.dtx  (with options: `hobby')
%% ----------------------------------------------------------------
%% hobby --- a TikZ/PGF library for drawing smooth(ish) curves using
%%           Hobby's algorithm (implemented in LaTeX3)
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\RequirePackage{expl3}
\RequirePackage{xparse}
\RequirePackage{pml3array}
\ExplSyntaxOn
\cs_generate_variant:Nn \fp_set:Nn {Nx}
\cs_generate_variant:Nn \tl_if_eq:nnTF {VnTF}
\cs_generate_variant:Nn \tl_if_eq:nnTF {xnTF}
\tl_clear:N \l_tmpa_tl
\tl_if_exist:NT \g__hobby_version
{
  \tl_set:Nn \l_tmpa_tl {
    \ExplSyntaxOff
    \tl_clear:N \l_tmpa_tl
    \endinput
  }
}
\tl_use:N \l_tmpa_tl

\tl_new:N \g__hobby_version
\tl_new:N \g__hobby_date
\tl_set:Nn \g__hobby_version {1.8}
\tl_set:Nn \g__hobby_date {2017-06-01}
\DeclareDocumentCommand \hobbyVersion {}
{
  \tl_use:N \g__hobby_version
}
\DeclareDocumentCommand \hobbyDate {}
{
  \tl_use:N \g__hobby_date
}
\fp_new:N \g_hobby_parama_fp
\fp_new:N \g_hobby_paramb_fp
\fp_new:N \g_hobby_paramc_fp
\fp_gset:Nn \g_hobby_parama_fp {2^.5}
\fp_gset:Nn \g_hobby_paramb_fp {1/16}
\fp_gset:Nn \g_hobby_paramc_fp {(3-5^.5)/2}
\bool_new:N \l_hobby_closed_bool
\bool_new:N \l_hobby_disjoint_bool
\bool_new:N \l_hobby_save_aux_bool
\bool_set_true:N \l_hobby_save_aux_bool
\DeclareDocumentCommand \HobbyDisableAux {}
{
  \bool_set_false:N \l_hobby_save_aux_bool
}
\array_new:N \l_hobby_points_array
\array_new:N \l_hobby_points_x_array
\array_new:N \l_hobby_points_y_array
\array_new:N \l_hobby_actions_array
\array_new:N \l_hobby_angles_array
\array_new:N \l_hobby_distances_array
\array_new:N \l_hobby_tension_out_array
\array_new:N \l_hobby_tension_in_array
\array_new:N \l_hobby_matrix_a_array
\array_new:N \l_hobby_matrix_b_array
\array_new:N \l_hobby_matrix_c_array
\array_new:N \l_hobby_matrix_d_array
\array_new:N \l_hobby_vector_u_array
\array_new:N \l_hobby_excess_angle_array
\array_new:N \l_hobby_psi_array
\array_new:N \l_hobby_theta_array
\array_new:N \l_hobby_phi_array
\array_new:N \l_hobby_sigma_array
\array_new:N \l_hobby_rho_array
\array_new:N \l_hobby_controla_array
\array_new:N \l_hobby_controlb_array
\fp_new:N \l_hobby_matrix_v_fp
\fp_new:N \l_hobby_tempa_fp
\fp_new:N \l_hobby_tempb_fp
\fp_new:N \l_hobby_tempc_fp
\fp_new:N \l_hobby_tempd_fp
\fp_new:N \l_hobby_temps_fp
\fp_new:N \l_hobby_in_curl_fp
\fp_set:Nn \l_hobby_in_curl_fp {1}
\fp_new:N \l_hobby_out_curl_fp
\fp_set:Nn \l_hobby_out_curl_fp {1}
\fp_new:N \l_hobby_in_angle_fp
\fp_set_eq:NN \l_hobby_in_angle_fp \c_inf_fp
\fp_new:N \l_hobby_out_angle_fp
\fp_set_eq:NN \l_hobby_out_angle_fp \c_inf_fp
\int_new:N \l_hobby_npoints_int
\int_new:N \l_hobby_draw_int
\keys_define:nn {hobby / read in all} {
  x .fp_set:N = \l_hobby_tempa_fp,
  y .fp_set:N = \l_hobby_tempb_fp,
  tension~out .fp_set:N = \l_hobby_tempc_fp,
  tension~in .fp_set:N = \l_hobby_tempd_fp,
  excess~angle .fp_set:N = \l_hobby_temps_fp,
  break .tl_set:N = \l_tmpb_tl,
  blank .tl_set:N = \l_tmpa_tl,
  tension .meta:n = { tension~out=#1, tension~in=#1 },
  break .default:n = false,
  blank .default:n = false,
  invert~soft~blanks .choice:,
  invert~soft~blanks / true .code:n = {
    \int_gset:Nn \l_hobby_draw_int {0}
  },
  invert~soft~blanks / false .code:n = {
    \int_gset:Nn \l_hobby_draw_int {1}
  },
  invert~soft~blanks .default:n = true,
  tension~out .default:n = 1,
  tension~in .default:n = 1,
  excess~angle .default:n = 0,
  in~angle .fp_gset:N = \l_hobby_in_angle_fp,
  out~angle .fp_gset:N = \l_hobby_out_angle_fp,
  in~curl .fp_gset:N = \l_hobby_in_curl_fp,
  out~curl .fp_gset:N = \l_hobby_out_curl_fp,
  closed .bool_gset:N = \l_hobby_closed_bool,
  closed .default:n = true,
  disjoint .bool_gset:N = \l_hobby_disjoint_bool,
  disjoint .default:n = true,
  break~default .code:n = {
    \keys_define:nn { hobby / read in all }
    {
      break .default:n = #1
    }
  },
  blank~default .code:n = {
    \keys_define:nn { hobby / read in all }
    {
      blank .default:n = #1
    }
  },
}
\keys_define:nn { hobby / read in params} {
  in~angle .fp_gset:N = \l_hobby_in_angle_fp,
  out~angle .fp_gset:N = \l_hobby_out_angle_fp,
  in~curl .fp_gset:N = \l_hobby_in_curl_fp,
  out~curl .fp_gset:N = \l_hobby_out_curl_fp,
  closed .bool_gset:N = \l_hobby_closed_bool,
  closed .default:n = true,
  disjoint .bool_gset:N = \l_hobby_disjoint_bool,
  disjoint .default:n = true,
  break~default .code:n = {
    \keys_define:nn { hobby / read in all }
    {
      break .default:n = #1
    }
  },
  blank~default .code:n = {
    \keys_define:nn { hobby / read in all }
    {
      blank .default:n = #1
    }
  },
  invert~soft~blanks .choice:,
  invert~soft~blanks / true .code:n = {
    \int_gset:Nn \l_hobby_draw_int {0}
  },
  invert~soft~blanks / false .code:n = {
    \int_gset:Nn \l_hobby_draw_int {1}
  },
  invert~soft~blanks .default:n = true,
}
\cs_set:Nn \hobby_distangle:n {
  \fp_set:Nn \l_hobby_tempa_fp {
    (\array_get:Nn \l_hobby_points_x_array {#1 + 1})
    - (\array_get:Nn \l_hobby_points_x_array {#1})}

  \fp_set:Nn \l_hobby_tempb_fp {
    (\array_get:Nn \l_hobby_points_y_array {#1 + 1})
    - (\array_get:Nn \l_hobby_points_y_array {#1})}

  \fp_set:Nn \l_hobby_tempc_fp { atan ( \l_hobby_tempb_fp, \l_hobby_tempa_fp ) }
  \fp_veclen:NVV \l_hobby_tempd_fp \l_hobby_tempa_fp \l_hobby_tempb_fp

  \array_push:Nx \l_hobby_angles_array {\fp_to_tl:N \l_hobby_tempc_fp}
  \array_push:Nx \l_hobby_distances_array {\fp_to_tl:N \l_hobby_tempd_fp}
  }
\cs_new:Nn \fp_veclen:Nnn {
  \fp_set:Nn #1 {((#2)^2 + (#3)^2)^.5}
}
\cs_generate_variant:Nn \fp_veclen:Nnn {NVV}
\cs_new:Nn \hobby_ctrllen:Nnn {
  \fp_set:Nn #1 {(2 - \g_hobby_parama_fp
    * ( sin(#2) - \g_hobby_paramb_fp * sin(#3) )
    * ( sin(#3) - \g_hobby_paramb_fp * sin(#2) )
    * ( cos(#2) - cos(#3) ) )
    / ( 1 + (1 - \g_hobby_paramc_fp) * cos(#3) + \g_hobby_paramc_fp * cos(#2))}
}
\cs_generate_variant:Nn \hobby_ctrllen:Nnn {NVV}
\cs_new_protected:Npn \hobby_append_point_copy:n #1
  {
    \hobby_append_point_copy_aux:Nn \l_hobby_points_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_points_x_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_points_y_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_tension_in_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_tension_out_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_excess_angle_array {#1}
    \hobby_append_point_copy_aux:Nn \l_hobby_actions_array {#1}
  }
\cs_new_protected:Npn \hobby_append_point_copy_aux:Nn #1#2
  { \array_gpush:Nx #1 { \array_get:Nn #1 {#2} } }
\cs_new:Nn \hobby_gen_path:
{
\bool_if:NT \l_hobby_closed_bool {
  \fp_compare:nTF {(\array_get:Nn \l_hobby_points_x_array {0})
    =
    (\array_top:N \l_hobby_points_x_array)}
  {
    \fp_compare:nF {
      \array_get:Nn \l_hobby_points_y_array {0}
      =
      \array_top:N \l_hobby_points_y_array
    }
  {
    \hobby_append_point_copy:n {0}
  }
  }
  {
    \hobby_append_point_copy:n {0}
  }
    \hobby_append_point_copy:n {1}
}
\int_gset:Nn \l_hobby_npoints_int {\array_length:N \l_hobby_points_y_array}
\int_compare:nNnTF {\l_hobby_npoints_int} = {0} {
}
{
  \int_compare:nNnTF {\l_hobby_npoints_int} = {1} {
\hobby_distangle:n {0}
\fp_compare:nF { \l_hobby_out_angle_fp == \c_inf_fp }
{
  \fp_set:Nn \l_hobby_tempa_fp { \l_hobby_out_angle_fp
    - \array_get:Nn \l_hobby_angles_array {0}}
    \fp_compare:nT {\l_hobby_tempa_fp > \c_pi_fp }
    {
      \fp_sub:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
    \fp_compare:nT {\l_hobby_tempa_fp < -\c_pi_fp }
    {
      \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
  \array_put:Nnx \l_hobby_theta_array {0} {\fp_to_tl:N \l_hobby_tempa_fp}
    \fp_compare:nT { \l_hobby_in_angle_fp == \c_inf_fp }
    {
      \array_put:Nnx \l_hobby_phi_array {1}{ \fp_to_tl:N \l_hobby_tempa_fp}
    }
   }
\fp_compare:nTF { \l_hobby_in_angle_fp == \c_inf_fp }
{
  \fp_compare:nT { \l_hobby_out_angle_fp == \c_inf_fp }
  {
    \array_put:Nnx \l_hobby_phi_array {1} {0}
    \array_put:Nnx \l_hobby_theta_array {0} {0}
  }
}
{
  \fp_set:Nn \l_hobby_tempa_fp { - \l_hobby_in_angle_fp + \c_pi_fp
+ (\array_get:Nn \l_hobby_angles_array {0})}
  \fp_compare:nT {\l_hobby_tempa_fp > \c_pi_fp }
  {
    \fp_sub:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
  }
  \fp_compare:nT {\l_hobby_tempa_fp < -\c_pi_fp }
  {
    \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
  }

  \array_put:Nnx \l_hobby_phi_array {1}
  {\fp_to_tl:N \l_hobby_tempa_fp}
  \fp_compare:nT { \l_hobby_out_angle_fp == \c_inf_fp }
    {
      \array_put:Nnx \l_hobby_theta_array {0}{ \fp_to_tl:N \l_hobby_tempa_fp}
    }
}

  }
  {
    \hobby_compute_path:
  }
  \hobby_build_path:
}
}
\cs_new:Nn \hobby_compute_path:
{
\int_step_function:nnnN {0} {1} {\l_hobby_npoints_int - 1} \hobby_distangle:n
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 1} {
    \fp_set:Nx \l_hobby_tempa_fp {
    \array_get:Nn \l_hobby_angles_array {##1}
    - \array_get:Nn \l_hobby_angles_array {##1 - 1}}
    \fp_compare:nTF {\l_hobby_tempa_fp > \c_pi_fp }
    {
      \fp_sub:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
    {}
    \fp_compare:nTF {\l_hobby_tempa_fp <= -\c_pi_fp }
    {
      \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
    {}
\array_get:NnNTF \l_hobby_excess_angle_array {##1} \l_tmpa_tl {
  \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp * \l_tmpa_tl}
  }{}
    \array_put:Nnx \l_hobby_psi_array {##1}{\fp_to_tl:N \l_hobby_tempa_fp}
  }
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 1} {
    \array_put:Nnx \l_hobby_matrix_a_array {##1} {\fp_to_tl:n {
       \array_get:Nn \l_hobby_tension_in_array {##1}^2
      * \array_get:Nn \l_hobby_distances_array {##1}
      * \array_get:Nn \l_hobby_tension_in_array {##1 + 1}
  }}
}
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 1} {

  \array_put:Nnx \l_hobby_matrix_b_array {##1} {\fp_to_tl:n
{(3 * (\array_get:Nn \l_hobby_tension_in_array {##1 + 1}) - 1) *
 (\array_get:Nn \l_hobby_tension_out_array {##1})^2 *
(\array_get:Nn \l_hobby_tension_out_array {##1 - 1})
* ( \array_get:Nn \l_hobby_distances_array {##1 - 1})
+
(3 * (\array_get:Nn \l_hobby_tension_out_array {##1 - 1}) - 1)
* (\array_get:Nn \l_hobby_tension_in_array {##1})^2
* (\array_get:Nn \l_hobby_tension_in_array {##1 + 1})
* (\array_get:Nn \l_hobby_distances_array {##1})}
}
}
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 2} {

  \array_put:Nnx \l_hobby_matrix_c_array {##1} {\fp_to_tl:n
{(\array_get:Nn \l_hobby_tension_in_array {##1})^2
* (\array_get:Nn \l_hobby_tension_in_array {##1 - 1})
* (\array_get:Nn \l_hobby_distances_array {##1 - 1})
}}

}
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 2} {

  \array_put:Nnx \l_hobby_matrix_d_array {##1} {\fp_to_tl:n
{
- (\array_get:Nn \l_hobby_psi_array {##1 + 1})
* (\array_get:Nn \l_hobby_tension_out_array {##1})^2
* (\array_get:Nn \l_hobby_tension_out_array {##1 - 1})
* (\array_get:Nn \l_hobby_distances_array {##1 - 1})
- (3 * (\array_get:Nn \l_hobby_tension_out_array {##1 - 1}) - 1)
* (\array_get:Nn \l_hobby_psi_array {##1})
* (\array_get:Nn \l_hobby_tension_in_array {##1})^2
* (\array_get:Nn \l_hobby_tension_in_array {##1 + 1})
* (\array_get:Nn \l_hobby_distances_array {##1})
}
}
}
\bool_if:NTF \l_hobby_closed_bool {
\array_put:Nnx \l_hobby_matrix_c_array {0} {\fp_to_tl:n {
- (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int - 2})
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2})
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^2
}}

\array_put:Nnn \l_hobby_matrix_b_array {0} {1}
\array_put:Nnn \l_hobby_matrix_d_array {0} {0}

\array_put:Nnx \l_hobby_matrix_b_array {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
(\array_get:Nn \l_hobby_matrix_b_array {\l_hobby_npoints_int - 1})
+ 1
}}

 \array_put:Nnx \l_hobby_matrix_d_array {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
- (\array_get:Nn \l_hobby_psi_array {1})
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int -1})^2
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int -2})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int - 2})
- (3 * (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2}) - 1)
* (\array_get:Nn \l_hobby_psi_array {\l_hobby_npoints_int - 1})
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int - 1})^2
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int -1})
}
}
  \array_put:Nnn \l_hobby_vector_u_array {0} {1}
\array_put:Nnn \l_hobby_vector_u_array {\l_hobby_npoints_int - 1} {1}
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 2} {
  \array_put:Nnn \l_hobby_vector_u_array {##1} {0}
  }
\fp_set:Nn \l_hobby_matrix_v_fp {
(\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int -1})^2
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int -2})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int -2})
}
}
{
\fp_compare:nTF { \l_hobby_out_angle_fp == \c_inf_fp }
{
  \array_put:Nnx \l_hobby_matrix_b_array {0}  {\fp_to_tl:n {
  (\array_get:Nn \l_hobby_tension_in_array {1})^3
* \l_hobby_in_curl_fp
+
(3 * (\array_get:Nn \l_hobby_tension_in_array {1}) - 1)
* (\array_get:Nn \l_hobby_tension_out_array {0})^3
}}

  \array_put:Nnx \l_hobby_matrix_c_array {0} {\fp_to_tl:n {
  (\array_get:Nn \l_hobby_tension_out_array {0})^3
+
(3 * (\array_get:Nn \l_hobby_tension_out_array {0}) - 1)
* (\array_get:Nn \l_hobby_tension_in_array {1})^3
* \l_hobby_in_curl_fp
}}

  \array_put:Nnx \l_hobby_matrix_d_array {0} {\fp_to_tl:n {
-(  (\array_get:Nn \l_hobby_tension_out_array {0})^3
+
(3 * (\array_get:Nn \l_hobby_tension_out_array {0}) - 1)
* (\array_get:Nn \l_hobby_tension_in_array {1})^3
* \l_hobby_in_curl_fp)
* (\array_get:Nn \l_hobby_psi_array {1})
}}

}
{
  \array_put:Nnn \l_hobby_matrix_b_array {0} {1}
  \array_put:Nnn \l_hobby_matrix_c_array {0} {0}
  \fp_set:Nn \l_hobby_tempa_fp { \l_hobby_out_angle_fp
    - \array_get:Nn \l_hobby_angles_array {0}}
    \fp_compare:nT {\l_hobby_tempa_fp > \c_pi_fp }
    {
      \fp_sub:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
    \fp_compare:nT {\l_hobby_tempa_fp < -\c_pi_fp }
    {
      \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
    }
  \array_put:Nnx \l_hobby_matrix_d_array {0} {\fp_to_tl:N \l_hobby_tempa_fp}
}
\fp_compare:nTF { \l_hobby_in_angle_fp == \c_inf_fp }
{

 \array_put:Nnx \l_hobby_matrix_b_array {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
\array_get:Nn \l_hobby_matrix_b_array {\l_hobby_npoints_int - 1}
- (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^2
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int - 2})
*
((3 * (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int} ) - 1)
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^3 \l_tmpa_tl
* \l_hobby_out_curl_fp
+
(\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int })^3)
/
((3 * (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int -2}) - 1)
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int})^3
+
( \array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^3
* \l_hobby_out_curl_fp)
}}

 \array_put:Nnx \l_hobby_matrix_d_array {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
- (3 * (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2}) - 1)
* (\array_get:Nn \l_hobby_psi_array {\l_hobby_npoints_int - 1})
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int - 1})^2
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int - 1})
}}

}
{
  \fp_set:Nn \l_hobby_tempa_fp { - \l_hobby_in_angle_fp + \c_pi_fp
+ (\array_get:Nn \l_hobby_angles_array {\l_hobby_npoints_int - 1})}
  \fp_compare:nT {\l_hobby_tempa_fp > \c_pi_fp }
  {
    \fp_sub:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
  }
  \fp_compare:nT {\l_hobby_tempa_fp < -\c_pi_fp }
  {
    \fp_add:Nn \l_hobby_tempa_fp {2 * \c_pi_fp}
  }

  \array_put:Nnx \l_hobby_phi_array {\l_hobby_npoints_int}
  {\fp_to_tl:N \l_hobby_tempa_fp}

   \array_put:Nnx \l_hobby_matrix_d_array  {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
 \l_hobby_tempa_fp
 * (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^2
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2})
* (\array_get:Nn \l_hobby_distances_array {\l_hobby_npoints_int - 2})
-
(3 * ( \array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 2}) - 1)
* (\array_get:Nn \l_hobby_psi_array {\l_hobby_npoints_int - 1})
* (\array_get:Nn \l_hobby_tension_in_array  {\l_hobby_npoints_int - 1})^2
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int})
* (\array_get:Nn \l_hobby_distances_array  {\l_hobby_npoints_int - 1}) }}
}
}
\int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 1} {

  \array_put:Nnx \l_hobby_matrix_b_array {##1} {\fp_to_tl:n {
  (\array_get:Nn \l_hobby_matrix_b_array {##1 - 1})
* (\array_get:Nn \l_hobby_matrix_b_array {##1})
-
(\array_get:Nn \l_hobby_matrix_c_array {##1 - 1})
* (\array_get:Nn \l_hobby_matrix_a_array {##1})
}}
  \int_compare:nT {##1 < \l_hobby_npoints_int - 1} {

  \array_put:Nnx \l_hobby_matrix_c_array {##1} {\fp_to_tl:n {
(\array_get:Nn \l_hobby_matrix_b_array {##1 - 1})
    * (\array_get:Nn \l_hobby_matrix_c_array {##1})
}}
  }

  \array_put:Nnx \l_hobby_matrix_d_array {##1} {\fp_to_tl:n {
(\array_get:Nn \l_hobby_matrix_b_array {##1 - 1})
  * (\array_get:Nn \l_hobby_matrix_d_array {##1})
-
  (\array_get:Nn \l_hobby_matrix_d_array {##1 - 1})
  * (\array_get:Nn \l_hobby_matrix_a_array {##1})
}}
  \bool_if:NT \l_hobby_closed_bool {
  \array_put:Nnx \l_hobby_vector_u_array {##1} {\fp_to_tl:n {
(\array_get:Nn \l_hobby_matrix_b_array {##1 - 1})
* (\array_get:Nn \l_hobby_vector_u_array {##1})
-
(\array_get:Nn \l_hobby_vector_u_array {##1 - 1})
* (\array_get:Nn \l_hobby_matrix_a_array {##1})
}}
}
}
 \array_put:Nnx \l_hobby_theta_array  {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
(\array_get:Nn \l_hobby_matrix_d_array  {\l_hobby_npoints_int - 1})
/ (\array_get:Nn \l_hobby_matrix_b_array  {\l_hobby_npoints_int - 1})
}}
\bool_if:NT \l_hobby_closed_bool {
 \array_put:Nnx \l_hobby_vector_u_array  {\l_hobby_npoints_int - 1} {\fp_to_tl:n {
  (\array_get:Nn \l_hobby_vector_u_array  {\l_hobby_npoints_int - 1})
/ (\array_get:Nn \l_hobby_matrix_b_array  {\l_hobby_npoints_int - 1})
}}
}
\int_step_inline:nnnn {\l_hobby_npoints_int - 2} {-1} {0} {

  \array_put:Nnx \l_hobby_theta_array {##1} {\fp_to_tl:n {
( (\array_get:Nn \l_hobby_matrix_d_array {##1})
  - (\array_get:Nn \l_hobby_theta_array  {##1 + 1})
  * (\array_get:Nn \l_hobby_matrix_c_array {##1})
) / (\array_get:Nn \l_hobby_matrix_b_array {##1})
}}
}
\bool_if:NT \l_hobby_closed_bool {
\int_step_inline:nnnn {\l_hobby_npoints_int - 2} {-1} {0} {
  \array_put:Nnx \l_hobby_vector_u_array {##1} {\fp_to_tl:n
{
    ((\array_get:Nn \l_hobby_vector_u_array {##1})
    - (\array_get:Nn \l_hobby_vector_u_array  {##1 + 1})
    * (\array_get:Nn \l_hobby_matrix_c_array {##1})
    ) / (\array_get:Nn \l_hobby_matrix_b_array {##1})
}}
}

\fp_set:Nn \l_hobby_tempb_fp {
((\array_get:Nn \l_hobby_theta_array {1})
* \l_hobby_matrix_v_fp
- (\array_get:Nn \l_hobby_theta_array  {\l_hobby_npoints_int - 1})
) / (
(\array_get:Nn \l_hobby_vector_u_array {1})
* \l_hobby_matrix_v_fp
- (\array_get:Nn \l_hobby_vector_u_array  {\l_hobby_npoints_int - 1})
+ 1
)}

\int_step_inline:nnnn {0} {1} {\l_hobby_npoints_int - 1} {

  \array_put:Nnx \l_hobby_theta_array {##1} {\fp_to_tl:n {
  (\array_get:Nn \l_hobby_theta_array {##1})
  - (\array_get:Nn \l_hobby_vector_u_array {##1})
  * \l_hobby_tempb_fp
}}
}
}
\int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int - 1} {

    \array_put:Nnx \l_hobby_phi_array {##1} {\fp_to_tl:n {
      - (\array_get:Nn \l_hobby_psi_array {##1})
      - (\array_get:Nn \l_hobby_theta_array {##1})
  }}
  }
\bool_if:NTF \l_hobby_closed_bool {
  \int_gdecr:N \l_hobby_npoints_int
}{
\fp_compare:nT { \l_hobby_in_angle_fp == \c_inf_fp }
{
 \array_put:Nnx \l_hobby_phi_array {\l_hobby_npoints_int} {\fp_to_tl:n {
((3 * (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int}) - 1)
* (\array_get:Nn \l_hobby_tension_out_array {\l_hobby_npoints_int - 1})^3
* \l_hobby_out_curl_fp
+
(\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int })^3)
/
((3 * (\array_get:Nn \l_hobby_tension_out_array  {\l_hobby_npoints_int -2}) - 1)
* (\array_get:Nn \l_hobby_tension_in_array {\l_hobby_npoints_int})^3 \l_tmpa_tl
+
(\array_get:Nn \l_hobby_tension_out_array  {\l_hobby_npoints_int - 1})^3
* \l_hobby_out_curl_fp)
*
(\array_get:Nn \l_hobby_theta_array  {\l_hobby_npoints_int -1})
}}
}
}
}
\cs_new:Nn \hobby_build_path:
{
\int_step_inline:nnnn {0} {1} {\l_hobby_npoints_int - 1} {

  \fp_set:Nn \l_hobby_tempa_fp {\array_get:Nn \l_hobby_theta_array {##1}}

  \fp_set:Nn \l_hobby_tempb_fp {\array_get:Nn \l_hobby_phi_array  {##1 + 1}}

  \hobby_ctrllen:NVV \l_hobby_temps_fp \l_hobby_tempa_fp \l_hobby_tempb_fp

   \array_put:Nnx \l_hobby_sigma_array {##1 + 1} {\fp_to_tl:N \l_hobby_temps_fp}

  \hobby_ctrllen:NVV \l_hobby_temps_fp \l_hobby_tempb_fp \l_hobby_tempa_fp

   \array_put:Nnx \l_hobby_rho_array {##1} {\fp_to_tl:N \l_hobby_temps_fp}

  }
\int_step_inline:nnnn {0} {1} {\l_hobby_npoints_int - 1} {
\array_gput:Nnx \l_hobby_controla_array  {##1 + 1} {x = \fp_eval:n  {
(\array_get:Nn \l_hobby_points_x_array {##1})
+
  (\array_get:Nn \l_hobby_distances_array {##1}) *
  (\array_get:Nn \l_hobby_rho_array {##1}) *
cos ( (\array_get:Nn \l_hobby_angles_array {##1})
+
  (\array_get:Nn \l_hobby_theta_array {##1}))
/3
}, y = \fp_eval:n {
( \array_get:Nn \l_hobby_points_y_array {##1}) +
  (\array_get:Nn \l_hobby_distances_array {##1}) *
  (\array_get:Nn \l_hobby_rho_array {##1}) *
sin ( (\array_get:Nn \l_hobby_angles_array {##1})
+
  (\array_get:Nn \l_hobby_theta_array {##1}))
/3
}
}
}
\int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int} {
  \array_gput:Nnx \l_hobby_controlb_array {##1} {
    x = \fp_eval:n {\array_get:Nn \l_hobby_points_x_array {##1}
- (\array_get:Nn \l_hobby_distances_array  {##1 - 1})
* (\array_get:Nn \l_hobby_sigma_array {##1})
* cos((\array_get:Nn \l_hobby_angles_array  {##1 - 1})
- (\array_get:Nn \l_hobby_phi_array {##1}))/3
}, y = \fp_eval:n {
  (\array_get:Nn \l_hobby_points_y_array {##1})
- (\array_get:Nn \l_hobby_distances_array  {##1 - 1})
* (\array_get:Nn \l_hobby_sigma_array {##1})
* sin((\array_get:Nn \l_hobby_angles_array  {##1 - 1})
- (\array_get:Nn \l_hobby_phi_array {##1}))/3
} }
 }
}
\NewDocumentCommand \hobbyinit {m m m} {
  \hobby_set_cmds:nnn#1#2#3
  \hobby_clear_path:
}
\NewDocumentCommand \hobbyaddpoint { m } {
    \keys_set:nn { hobby/read in all }
    {
      tension~out,
      tension~in,
      excess~angle,
      blank,
      break,
      #1
    }
    \tl_if_eq:VnTF {\l_tmpa_tl} {true}
     {\tl_set:Nn \l_tmpa_tl {2}}
     {
       \tl_if_eq:VnTF {\l_tmpa_tl} {soft}
       {\tl_set:Nn \l_tmpa_tl {0}}
       {\tl_set:Nn \l_tmpa_tl {1}}
     }
    \tl_if_eq:VnTF {\l_tmpb_tl} {true}
     {\tl_put_right:Nn \l_tmpa_tl {1}}
     {\tl_put_right:Nn \l_tmpa_tl {0}}
    \array_gpush:Nx \l_hobby_actions_array {\l_tmpa_tl}
    \array_gpush:Nx \l_hobby_tension_out_array {\fp_to_tl:N \l_hobby_tempc_fp}
    \array_gpush:Nx \l_hobby_tension_in_array {\fp_to_tl:N \l_hobby_tempd_fp}
    \array_gpush:Nx \l_hobby_excess_angle_array {\fp_to_tl:N \l_hobby_temps_fp}
    \array_gpush:Nx \l_hobby_points_array {
      x = \fp_use:N \l_hobby_tempa_fp,
      y = \fp_use:N \l_hobby_tempb_fp }
    \array_gpush:Nx \l_hobby_points_x_array {\fp_to_tl:N \l_hobby_tempa_fp}
    \array_gpush:Nx \l_hobby_points_y_array {\fp_to_tl:N \l_hobby_tempb_fp}
}
\NewDocumentCommand \hobbysetparams { m } {
  \keys_set:nn { hobby / read in params }
  {
    #1
  }
}
\cs_new:Npn \hobby_moveto:nnn #1#2#3 {}
\cs_new:Npn \hobby_curveto:nnn #1#2#3 {}
\cs_new:Npn \hobby_close:n #1 {}
\cs_generate_variant:Nn \hobby_moveto:nnn {VVV,nnV}
\cs_generate_variant:Nn \hobby_curveto:nnn {VVV}
\cs_generate_variant:Nn \hobby_close:n {V}
\cs_new:Nn \hobby_set_cmds:nnn {
  \cs_gset_eq:NN \hobby_moveto:nnn #1
  \cs_gset_eq:NN \hobby_curveto:nnn #2
  \cs_gset_eq:NN \hobby_close:n #3
}
\NewDocumentCommand \hobbygenpath { } {
  \array_if_empty:NF \l_hobby_points_array {
    \hobby_gen_path:
  }
}
\NewDocumentCommand \hobbygenifnecpath { m } {
  \tl_if_exist:cTF {g_hobby_#1_path}
  {
    \tl_use:c {g_hobby_#1_path}
  }
  {
    \hobby_gen_path:
  }
  \hobby_save_path:n {#1}
  \hobby_save_path_to_aux:x {#1}
}
\NewDocumentCommand \hobbygenuseifnecpath { m } {
  \tl_if_exist:cTF {g_hobby_#1_path}
  {
    \tl_use:c {g_hobby_#1_path}
  }
  {
    \hobby_gen_path:
  }
  \hobby_save_path:n {#1}
  \hobby_save_path_to_aux:x {#1}
  \hobby_use_path:
}
\NewDocumentCommand \hobbyusepath { m } {
  \hobbysetparams{#1}
  \hobby_use_path:
}
\NewDocumentCommand \hobbysavepath { m } {
  \hobby_save_path:n {#1}
}
\NewDocumentCommand \hobbyrestorepath { m } {
  \tl_if_exist:cT {g_hobby_#1_path} {
    \tl_use:c {g_hobby_#1_path}
  }
}
\NewDocumentCommand \hobbyshowpath { m } {
  \tl_if_exist:cT {g_hobby_#1_path} {
    \tl_show:c {g_hobby_#1_path}
  }
}
\NewDocumentCommand \hobbygenusepath { } {
  \array_if_empty:NF \l_hobby_points_array {
    \hobby_gen_path:
    \hobby_use_path:
  }
}
\NewDocumentCommand \hobbyclearpath { } {
  \hobby_clear_path:
}
\tl_new:N \l_tmpc_tl
\cs_new:Nn \hobby_use_path: {
  \bool_if:NT \l_hobby_disjoint_bool {
    \array_get:NnN \l_hobby_points_array {0} \l_tmpa_tl
    \hobby_moveto:nnV {} {} \l_tmpa_tl
  }
  \int_step_inline:nnnn {1} {1} {\l_hobby_npoints_int} {
    \array_get:NnN \l_hobby_controla_array {##1} \l_tmpa_tl
    \array_get:NnN \l_hobby_controlb_array {##1} \l_tmpb_tl
    \array_get:NnN \l_hobby_points_array {##1} \l_tmpc_tl
    \array_get:NnN \l_hobby_actions_array {##1} \l_tmpd_tl
    \int_compare:nNnTF {\tl_item:Nn \l_tmpd_tl {1}} = {\l_hobby_draw_int} {
      \hobby_curveto:VVV \l_tmpa_tl \l_tmpb_tl \l_tmpc_tl
    }{
      \bool_gset_false:N \l_hobby_closed_bool
      \hobby_moveto:VVV \l_tmpa_tl \l_tmpb_tl \l_tmpc_tl
    }
    \tl_if_eq:xnTF {\tl_item:Nn \l_tmpd_tl {2}} {1} {
      \bool_gset_false:N \l_hobby_closed_bool
      \hobby_moveto:VVV \l_tmpa_tl \l_tmpb_tl \l_tmpc_tl
    }{}
  }
  \bool_if:NT \l_hobby_closed_bool {
    \array_get:NnN \l_hobby_points_array {0} \l_tmpa_tl
    \hobby_close:V \l_tmpa_tl
  }
}
\cs_new:Nn \hobby_save_path:n {
  \tl_clear:N \l_tmpa_tl
  \tl_put_right:Nn \l_tmpa_tl {\int_gset:Nn \l_hobby_npoints_int}
  \tl_put_right:Nx \l_tmpa_tl {{\int_use:N \l_hobby_npoints_int}}
  \bool_if:NTF \l_hobby_disjoint_bool {
    \tl_put_right:Nn \l_tmpa_tl {\bool_gset_true:N}
  }{
    \tl_put_right:Nn \l_tmpa_tl {\bool_gset_false:N}
  }
  \tl_put_right:Nn \l_tmpa_tl {\l_hobby_disjoint_bool}
  \bool_if:NTF \l_hobby_closed_bool {
    \tl_put_right:Nn \l_tmpa_tl {\bool_gset_true:N}
  }{
    \tl_put_right:Nn \l_tmpa_tl {\bool_gset_false:N}
  }
  \tl_put_right:Nn \l_tmpa_tl {\l_hobby_closed_bool}
  \tl_put_right:Nn \l_tmpa_tl {\array_gclear:N \l_hobby_points_array}
  \array_map_inline:Nn \l_hobby_points_array {
    \tl_put_right:Nn \l_tmpa_tl {
      \array_gput:Nnn \l_hobby_points_array {##1} {##2}
    }
  }
  \tl_put_right:Nn \l_tmpa_tl {\array_gclear:N \l_hobby_actions_array}
  \array_map_inline:Nn \l_hobby_actions_array {
    \tl_put_right:Nn \l_tmpa_tl {
      \array_gput:Nnn \l_hobby_actions_array {##1} {##2}
    }
  }
  \tl_put_right:Nn \l_tmpa_tl {\array_gclear:N \l_hobby_controla_array}
  \array_map_inline:Nn \l_hobby_controla_array {
    \tl_put_right:Nn \l_tmpa_tl {
      \array_gput:Nnn \l_hobby_controla_array {##1} {##2}
    }
  }
  \tl_put_right:Nn \l_tmpa_tl {\array_gclear:N \l_hobby_controlb_array}
  \array_map_inline:Nn \l_hobby_controlb_array {
    \tl_put_right:Nn \l_tmpa_tl {
      \array_gput:Nnn \l_hobby_controlb_array {##1} {##2}
    }
  }
  \tl_gclear_new:c {g_hobby_#1_path}
  \tl_gset_eq:cN {g_hobby_#1_path} \l_tmpa_tl
}
\int_set:Nn \l_tmpa_int {\char_value_catcode:n {`@}}
\char_set_catcode_letter:N @
\cs_new:Npn \hobby_save_path_to_aux:n #1 {
  \bool_if:nT {
    \tl_if_exist_p:c {g_hobby_#1_path}
    &&
    ! \tl_if_exist_p:c {g_hobby_#1_path_saved}
    &&
    \l_hobby_save_aux_bool
  }
  {
    \tl_clear:N \l_tmpa_tl
    \tl_put_right:Nn \l_tmpa_tl {
      \ExplSyntaxOn
      \tl_gclear_new:c {g_hobby_#1_path}
      \tl_gput_right:cn {g_hobby_#1_path}
    }
    \tl_put_right:Nx \l_tmpa_tl {
      {\tl_to_str:c {g_hobby_#1_path}}
    }
    \tl_put_right:Nn \l_tmpa_tl {
      \ExplSyntaxOff
    }
    \protected@write\@auxout{}{
      \tl_to_str:N \l_tmpa_tl
    }
    \tl_new:c {g_hobby_#1_path_saved}
  }
}
\char_set_catcode:nn {`@} {\l_tmpa_int}
\cs_generate_variant:Nn \hobby_save_path_to_aux:n {x}
\cs_new:Nn \hobby_clear_path:
{
\array_gclear:N \l_hobby_points_array
\array_gclear:N \l_hobby_points_x_array
\array_gclear:N \l_hobby_points_y_array
\array_gclear:N \l_hobby_angles_array
\array_gclear:N \l_hobby_actions_array
\array_gclear:N \l_hobby_distances_array
\array_gclear:N \l_hobby_tension_out_array
\array_gclear:N \l_hobby_tension_in_array
\array_gclear:N \l_hobby_excess_angle_array
\array_gclear:N \l_hobby_matrix_a_array
\array_gclear:N \l_hobby_matrix_b_array
\array_gclear:N \l_hobby_matrix_c_array
\array_gclear:N \l_hobby_matrix_d_array
\array_gclear:N \l_hobby_vector_u_array
\array_gclear:N \l_hobby_psi_array
\array_gclear:N \l_hobby_theta_array
\array_gclear:N \l_hobby_phi_array
\array_gclear:N \l_hobby_sigma_array
\array_gclear:N \l_hobby_rho_array
\array_gclear:N \l_hobby_controla_array
\array_gclear:N \l_hobby_controlb_array
\bool_gset_false:N \l_hobby_closed_bool
\bool_gset_false:N \l_hobby_disjoint_bool

  \int_gset:Nn \l_hobby_npoints_int {-1}
  \int_gset:Nn \l_hobby_draw_int {1}
  \fp_gset_eq:NN \l_hobby_in_angle_fp \c_inf_fp
  \fp_gset_eq:NN \l_hobby_out_angle_fp \c_inf_fp
  \fp_gset_eq:NN \l_hobby_in_curl_fp \c_one_fp
  \fp_gset_eq:NN \l_hobby_out_curl_fp \c_one_fp
}
\ExplSyntaxOff
%% 
%% Copyright (C) 2012 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This file may be distributed and/or modified under the conditions
%% of the LaTeX Project Public License, either version 1.3 of this
%% license or (at your option) any later version.
%% The latest version of this license is in:
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  hobby.dtx
%%                                  hobby_doc.tex
%% and the derived files            hobby.code.tex
%%                                  pgflibraryhobby.code.tex
%%                                  tikzlibraryhobby.code.tex
%%                                  pml3array.sty
%%                                  hobby.ins
%%                                  hobby.pdf
%%                                  hobby_code.pdf
%%                                  README.txt
%% 
%%
%% End of file `hobby.code.tex'.


==> pgflibraryhobby.code.tex <==
%%
%% This is file `pgflibraryhobby.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% hobby.dtx  (with options: `pgflibrary')
%% ----------------------------------------------------------------
%% hobby --- a TikZ/PGF library for drawing smooth(ish) curves using
%%           Hobby's algorithm (implemented in LaTeX3)
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\input{hobby.code.tex}
\pgfkeys{
  /pgf/hobby/.is family,
  /pgf/hobby/.cd,
  x/.code={\pgf@x=#1cm},
  y/.code={\pgf@y=#1cm}
}
\pgfmathparse{atan2(0,1)}
\def\hobby@temp{0.0}
\ifx\pgfmathresult\hobby@temp
  \pgfmathdeclarefunction{hobbyatan2}{2}{%
    \pgfmathatantwo@{#1}{#2}%
  }
\else
  \pgfmathdeclarefunction{hobbyatan2}{2}{%
    \pgfmathatantwo@{#2}{#1}%
  }
\fi
\def\hobby@curveto#1#2#3{%
  \pgfpathcurveto{\hobby@topgf{#1}}{\hobby@topgf{#2}}{\hobby@topgf{#3}}%
}
\def\hobby@moveto#1#2#3{%
  \pgfpathmoveto{\hobby@topgf{#3}}%
}
\def\hobby@topgf#1{%
    \pgfqkeys{/pgf/hobby}{#1}%
}
\def\hobby@close#1{%
  \pgfpathclose
}
\def\pgfpathhobby{%
  \pgfutil@ifnextchar\bgroup{\pgfpath@hobby}{\pgfpath@hobby{}}}
\def\pgfpath@hobby#1{%
  \hobbyinit\hobby@moveto\hobby@curveto\hobby@close
  \hobbysetparams{#1}%
  \pgfmathsetmacro\hobby@x{\the\pgf@path@lastx/1cm}%
  \pgfmathsetmacro\hobby@y{\the\pgf@path@lasty/1cm}%
  \hobbyaddpoint{x = \hobby@x, y = \hobby@y}%
}
\def\pgfpathhobbypt#1{%
  #1%
  \pgfmathsetmacro\hobby@x{\the\pgf@x/1cm}%
  \pgfmathsetmacro\hobby@y{\the\pgf@y/1cm}%
  \pgfutil@ifnextchar\bgroup{\pgfpathhobbyptparams}{\pgfpathhobbyptparams{}}%
}
\def\pgfpathhobbyptparams#1{%
  \hobbyaddpoint{#1,x = \hobby@x, y = \hobby@y}%
}
\def\pgfpathhobbyend{%
  \ifhobby@externalise
    \ifx\hobby@path@name\pgfutil@empty
      \hobbygenusepath
    \else
      \hobbygenuseifnecpath{\hobby@path@name}%
    \fi
  \else
    \hobbygenusepath
  \fi
  \ifx\hobby@path@name\pgfutil@empty
  \else
    \hobbysavepath{\hobby@path@name}%
  \fi
  \global\let\hobby@path@name=\pgfutil@empty
}
\def\pgfplothandlerhobby{%
  \def\pgf@plotstreamstart{%
    \hobbyinit\hobby@moveto\hobby@curveto\hobby@close
    \global\let\pgf@plotstreampoint=\pgf@plot@hobby@firstpt
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble
    \gdef\pgf@plotstreamend{%
      \ifhobby@externalise
       \ifx\hobby@path@name\pgfutil@empty
        \hobbygenusepath
       \else
        \hobbygenuseifnecpath{\hobby@path@name}%
       \fi
      \else
       \hobbygenusepath
      \fi
      \ifx\hobby@path@name\pgfutil@empty
      \else
       \hobbysavepath{\hobby@path@name}%
      \fi
      \global\let\hobby@path@name=\pgfutil@empty
    }%
    \let\tikz@scan@point@options=\pgfutil@empty
  }
}
\def\pgfplothandlerclosedhobby{%
  \def\pgf@plotstreamstart{%
    \hobbyinit\hobby@moveto\hobby@curveto\hobby@close
    \hobbysetparams{closed=true,disjoint=true}%
    \global\let\pgf@plotstreampoint=\pgf@plot@hobby@firstpt
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble
    \gdef\pgf@plotstreamend{%
      \ifhobby@externalise
       \ifx\hobby@path@name\pgfutil@empty
        \hobbygenusepath
       \else
        \hobbygenuseifnecpath{\hobby@path@name}%
       \fi
      \else
       \hobbygenusepath
      \fi
      \ifx\hobby@path@name\pgfutil@empty
      \else
       \hobbysavepath{\hobby@path@name}%
      \fi
      \global\let\hobby@path@name=\pgfutil@empty
    }%
  }
}
\def\pgf@plot@hobby@firstpt#1{%
  \pgf@plot@first@action{#1}%
  \pgf@plot@hobby@handler{#1}%
  \global\let\pgf@plotstreampoint=\pgf@plot@hobby@handler
}
\def\pgf@plot@hobby@handler#1{%
    #1%
    \pgfmathsetmacro\hobby@x{\the\pgf@x/1cm}%
    \pgfmathsetmacro\hobby@y{\the\pgf@y/1cm}%
    \hobbyaddpoint{x = \hobby@x, y = \hobby@y}%
  }
\def\pgfplothandlerquickhobby{%
  \def\pgf@plotstreamstart{%
    \global\let\hobby@quick@curveto=\pgfpathcurveto
    \global\let\pgf@plotstreampoint=\pgf@plot@qhobby@firstpt
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble
    \global\let\pgf@plotstreamend=\pgf@plot@qhobby@end
  }
}
\def\pgf@plot@qhobby@firstpt#1{%
  #1%
  \edef\hobby@temp{\noexpand\pgf@plot@first@action{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}\hobby@temp%
  \xdef\hobby@qpoints{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \gdef\hobby@qpointa{}%
  \gdef\hobby@angle{}%
  \global\let\pgf@plotstreampoint=\pgf@plot@qhobby@secondpt
}
\def\pgf@plot@qhobby@secondpt#1{%
  #1%
  \xdef\hobby@qpointa{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@qhobby@handler
}
\def\pgf@plot@qhobby@handler#1{%
  #1
  \edef\hobby@temp{\noexpand\hobby@quick@compute{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}\hobby@temp
  \global\let\hobby@qpointa=\hobby@qpointa
  \global\let\hobby@qpoints=\hobby@qpoints
  \global\let\hobby@angle=\hobby@angle
  \global\let\hobby@thetaone=\hobby@thetaone
  \global\let\hobby@phitwo=\hobby@phitwo
  \global\let\hobby@done=\hobby@done
  \global\let\hobby@omegaone=\hobby@omegaone
}
\def\pgf@plot@qhobby@end{%
  \hobby@quick@computeend
}
\pgfmathsetmacro\hobby@sf{10cm}
\def\hobby@quick@compute#1{%
  #1%
  \pgf@xb=\pgf@x
  \pgf@yb=\pgf@y
  \hobby@qpointa
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \advance\pgf@xb by -\pgf@xa
  \advance\pgf@yb by -\pgf@ya
  \pgfmathsetmacro\hobby@done{sqrt((\pgf@xb/\hobby@sf)^2 + (\pgf@yb/\hobby@sf)^2)}%
  \pgfmathsetmacro\hobby@omegaone{rad(hobbyatan2(\pgf@yb,\pgf@xb))}%
  \hobby@qpoints
  \advance\pgf@xa by -\pgf@x
  \advance\pgf@ya by -\pgf@y
  \pgfmathsetmacro\hobby@dzero{sqrt((\pgf@xa/\hobby@sf)^2 + (\pgf@ya/\hobby@sf)^2)}%
  \pgfmathsetmacro\hobby@omegazero{rad(hobbyatan2(\pgf@ya,\pgf@xa))}%
  \pgfmathsetmacro\hobby@psi{\hobby@omegaone - \hobby@omegazero}%
  \pgfmathsetmacro\hobby@psi{\hobby@psi > pi ? \hobby@psi - 2*pi : \hobby@psi}%
  \pgfmathsetmacro\hobby@psi{\hobby@psi < -pi ? \hobby@psi + 2*pi : \hobby@psi}%
  \ifx\hobby@angle\pgfutil@empty
  \pgfmathsetmacro\hobby@thetaone{-\hobby@psi * \hobby@done%
/(\hobby@done + \hobby@dzero)}%
  \pgfmathsetmacro\hobby@thetazero{-\hobby@psi - \hobby@thetaone}%
  \let\hobby@phione=\hobby@thetazero
  \let\hobby@phitwo=\hobby@thetaone
  \else
  \let\hobby@thetazero=\hobby@angle
  \pgfmathsetmacro\hobby@thetaone{%
  -(2 * \hobby@psi + \hobby@thetazero) * \hobby@done%
  / (2 * \hobby@done + \hobby@dzero)}%
  \pgfmathsetmacro\hobby@phione{-\hobby@psi - \hobby@thetaone}%
  \let\hobby@phitwo=\hobby@thetaone
  \fi
  \let\hobby@angle=\hobby@thetaone
  \hobby@quick@ctrlpts{\hobby@thetazero}{\hobby@phione}{\hobby@qpoints}{\hobby@qpointa}{\hobby@dzero}{\hobby@omegazero}%
  \edef\hobby@temp{\noexpand\hobby@quick@curveto{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
\hobby@temp
  \global\let\hobby@qpoints=\hobby@qpointa
  #1
  \xdef\hobby@qpointa{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\hobby@angle=\hobby@angle
  \global\let\hobby@phitwo=\hobby@phitwo
  \global\let\hobby@thetaone=\hobby@thetaone
\global\let\hobby@done=\hobby@done
\global\let\hobby@omegaone=\hobby@omegaone
}
\def\hobby@quick@computeend{%
  \hobby@quick@ctrlpts{\hobby@thetaone}{\hobby@phitwo}{\hobby@qpoints}{\hobby@qpointa}{\hobby@done}{\hobby@omegaone}%
  \edef\hobby@temp{\noexpand\hobby@quick@curveto{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
\hobby@temp
}%
\def\hobby@quick@ctrlpts#1#2#3#4#5#6{%
  \pgfmathsetmacro\hobby@alpha{%
    sqrt(2) * (sin(#1 r) - 1/16 * sin(#2 r))%
* (sin(#2 r) - 1/16 * sin(#1 r))%
 * (cos(#1 r) - cos(#2 r))}%
  \pgfmathsetmacro\hobby@rho{%
    (2 + \hobby@alpha)/(1 + (1 - (3 - sqrt(5))/2)%
 * cos(#1 r) + (3 - sqrt(5))/2 * cos(#2 r))}%
  \pgfmathsetmacro\hobby@sigma{%
    (2 - \hobby@alpha)/(1 + (1 - (3 - sqrt(5))/2)%
  * cos(#2 r) +  (3 - sqrt(5))/2 * cos(#1 r))}%
  #3%
  \pgf@xa=\pgf@x
  \pgf@ya=\pgf@y
  \pgfmathsetlength\pgf@xa{%
    \pgf@xa + #5 * \hobby@rho%
  * cos((#1 + #6) r)/3*\hobby@sf}%
  \pgfmathsetlength\pgf@ya{%
    \pgf@ya + #5 * \hobby@rho%
  * sin((#1 + #6) r)/3*\hobby@sf}%
  #4%
  \pgf@xb=\pgf@x
  \pgf@yb=\pgf@y
  \pgfmathsetlength\pgf@xb{%
    \pgf@xb - #5 * \hobby@sigma%
  * cos((-#2 + #6) r)/3*\hobby@sf}%
  \pgfmathsetlength\pgf@yb{%
    \pgf@yb - #5 * \hobby@sigma%
  * sin((-#2 + #6) r)/3*\hobby@sf}%
  #4%
}
%% 
%% Copyright (C) 2012 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This file may be distributed and/or modified under the conditions
%% of the LaTeX Project Public License, either version 1.3 of this
%% license or (at your option) any later version.
%% The latest version of this license is in:
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  hobby.dtx
%%                                  hobby_doc.tex
%% and the derived files            hobby.code.tex
%%                                  pgflibraryhobby.code.tex
%%                                  tikzlibraryhobby.code.tex
%%                                  pml3array.sty
%%                                  hobby.ins
%%                                  hobby.pdf
%%                                  hobby_code.pdf
%%                                  README.txt
%% 
%%
%% End of file `pgflibraryhobby.code.tex'.


==> tikzlibraryhobby.code.tex <==
%%
%% This is file `tikzlibraryhobby.code.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% hobby.dtx  (with options: `tikzlibrary')
%% ----------------------------------------------------------------
%% hobby --- a TikZ/PGF library for drawing smooth(ish) curves using
%%           Hobby's algorithm (implemented in LaTeX3)
%% E-mail: loopspace@mathforge.org
%% Released under the LaTeX Project Public License v1.3c or later
%% See http://www.latex-project.org/lppl.txt
%% ----------------------------------------------------------------
%% 
\usepgflibrary{hobby}
\let\hobby@this@opts=\pgfutil@empty
\let\hobby@next@opts=\pgfutil@empty
\let\hobby@action=\pgfutil@empty
\let\hobby@path@name=\pgfutil@empty
\newif\ifhobby@externalise
\def\hobby@point@options{}%
\tikzset{
  curve through/.style={
    to path={
      \pgfextra{
        \expandafter\curvethrough\expandafter[\hobby@next@opts]{%
          (\tikztostart) .. #1 .. (\tikztotarget)%
        }
      }
    }
  },
  tension in/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,tension in=#1}%
  },
  tension out/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,tension out=#1}%
  },
  tension/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,tension=#1}%
  },
  excess angle/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,excess angle=#1}%
  },
  break/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,break=#1}%
  },
  blank/.code = {%
    \expandafter\gdef\expandafter\hobby@point@options\expandafter%
    {\hobby@point@options,blank=#1}%
  },
  designated Hobby path/.initial={next},
  clear next Hobby path options/.code={%
    \gdef\hobby@next@opts{}%
  },
  clear this Hobby path options/.code={%
    \gdef\hobby@this@opts{}%
  },
  clear Hobby path options/.style={%
    clear \pgfkeysvalueof{/tikz/designated Hobby path} Hobby path options
  },
  add option to this Hobby path/.code={%
    \expandafter\gdef\expandafter\hobby@this@opts\expandafter{\hobby@this@opts#1,}%
  },
  add option to next Hobby path/.code={%
    \expandafter\gdef\expandafter\hobby@next@opts\expandafter{\hobby@next@opts#1,}%
  },
  add option to Hobby path/.style={%
    add option to \pgfkeysvalueof{/tikz/designated Hobby path} Hobby path={#1}%
  },
  closed/.style = {%
    add option to Hobby path={closed=#1,disjoint=#1}%
  },
  invert blank/.style = {%
    add option to Hobby path={invert blank=#1}%
  },
  closed/.default = true,
  blank/.default = true,
  break/.default = true,
  invert blank/.default = true,
  in angle/.code = {%
    \pgfmathparse{(#1)*pi/180}%
    \edef\@temp{in angle=\pgfmathresult,}%
    \pgfkeysalso{add option to Hobby path/.expand once=\@temp}%
  },
  out angle/.code = {%
    \pgfmathparse{(#1)*pi/180}%
    \edef\@temp{out angle=\pgfmathresult,}%
    \pgfkeysalso{add option to Hobby path/.expand once=\@temp}%
  },
  in curl/.style = {%
    add option to Hobby path={in curl=#1}%
  },
  out curl/.code = {%
    add option to Hobby path={out curl=#1}%
  },
  use Hobby shortcut/.code={%
    \let\tikz@curveto@auto=\hobby@curveto@override
    \global\let\hobby@curveto@delegate=\hobby@curveto@auto
  },
  use quick Hobby shortcut/.code={%
    \let\tikz@curveto@auto=\hobby@curveto@override
    \global\let\hobby@curveto@delegate=\hobby@qcurveto@auto
  },
  use previous Hobby path/.code={%
    \pgfextra{\hobbyusepath{#1}}
  },
  use previous Hobby path/.default={},%
  save Hobby path/.code={%
    \xdef\hobby@path@name{#1}%
  },
  restore Hobby path/.code={%
    \pgfextra{%
      \hobbyinit\hobby@tikz@moveto\hobby@tikz@curveto\hobby@tikz@close
      \global\let\hobby@collected@onpath\pgfutil@empty
      \hobbyrestorepath{#1}}
  },
  restore and use Hobby path/.code 2 args={%
    \pgfextra{%
      \hobbyinit\hobby@tikz@moveto\hobby@tikz@curveto\hobby@tikz@close
      \global\let\hobby@collected@onpath\pgfutil@empty
      \hobbyrestorepath{#1}%
      \hobbyusepath{#2}%
    }
  },
  show Hobby path/.code={%
    \pgfextra{\hobbyshowpath{#1}}
  },
  Hobby action/.code={%
    \expandafter\gdef\expandafter\hobby@action\expandafter{\hobby@action#1}%
  },
  Hobby finish/.style={%
    Hobby action=\hobby@finish%
  },
  Hobby externalise/.is if=hobby@externalise,
  Hobby externalize/.is if=hobby@externalise
}
\def\hobby@tikz@curveto#1#2#3{%
  \pgfutil@ifundefined{tikz@timer@start}{%
    \expandafter\hobby@topgf\expandafter{\hobby@initial@pt}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  }{}%
  \hobby@topgf{#1}%
  \edef\tikz@timer@cont@one{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \hobby@topgf{#2}%
  \edef\tikz@timer@cont@two{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \hobby@topgf{#3}%
  \let\tikz@timer=\tikz@timer@curve
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \ifx\hobby@collected@onpath\pgfutil@empty
  \else
  \expandafter\hobby@nodes@onpath\hobby@collected@onpath\relax\relax
  \fi
  \pgfpathcurveto{\hobby@topgf{#1}}{\hobby@topgf{#2}}{\hobby@topgf{#3}}%
  \hobby@topgf{#3}%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
}
\def\hobby@tikz@moveto#1#2#3{%
  \pgfutil@ifundefined{tikz@timer@start}{%
    \expandafter\hobby@topgf\expandafter{\hobby@initial@pt}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  }{}%
  \hobby@topgf{#3}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@timer=\tikz@timer@line
  \expandafter\def\expandafter\hobby@collected@onpath\expandafter{\expandafter{\expandafter}\hobby@collected@onpath}
  \else
    \hobby@topgf{#1}%
    \edef\tikz@timer@cont@one{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \hobby@topgf{#2}%
    \edef\tikz@timer@cont@two{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \let\tikz@timer=\tikz@timer@curve
  \fi
  \ifx\hobby@collected@onpath\pgfutil@empty
  \else
  \expandafter\hobby@nodes@onpath\hobby@collected@onpath\relax\relax
  \fi
  \pgfpathmoveto{\hobby@topgf{#3}}%
  \hobby@topgf{#3}%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
}
\def\hobby@tikz@close#1{%
  \hobby@topgf{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \let\tikz@timer=\tikz@timer@line
  \ifx\hobby@collected@onpath\pgfutil@empty
  \else
  \expandafter\hobby@nodes@onpath\hobby@collected@onpath\relax\relax
  \fi
  \pgfpathclose
}
\def\hobby@nodes@onpath#1#2\relax{%
  \gdef\hobby@collected@onpath{#2}%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty
  \else
  \def\@gtempa{\relax}
  \ifx\pgf@temp\@gtempa
  \else
  \tikz@node@is@a@labeltrue
  \tikz@scan@next@command#1\pgf@stop
  \tikz@node@is@a@labelfalse
  \fi
  \fi
}
\newcommand\curvethrough[2][]{%
  \hobbyinit\hobby@tikz@moveto\hobby@tikz@curveto\hobby@tikz@close
  \global\let\hobby@collected@onpath\pgfutil@empty
  \let\hobby@initial@pt\pgfutil@empty
  \hobbysetparams{#1}%
  \tikzset{designated Hobby path=this}%
  \global\let\hobby@this@opts=\pgfutil@empty
  \global\let\hobby@next@opts=\pgfutil@empty
  \let\tikz@scan@point@options=\pgfutil@empty
  \def\hobby@point@options{}%
  \tikz@scan@one@point\hobby@processpt #2 \relax%
}
\newcommand\hobby@processpt[1]{%
  #1%
  \pgfmathsetmacro\hobby@x{\the\pgf@x/1cm}%
  \pgfmathsetmacro\hobby@y{\the\pgf@y/1cm}%
  \ifx\hobby@initial@pt\pgfutil@empty
    \xdef\hobby@initial@pt{x = \hobby@x, y = \hobby@y}%
  \fi
  \expandafter\hobbyaddpoint\expandafter{\hobby@point@options,%
    x = \hobby@x, y = \hobby@y}%
  \def\hobby@point@options{}%
  \let\tikz@scan@point@options=\pgfutil@empty
  \pgfutil@ifnextchar\relax{%
    \expandafter\hobbysetparams\expandafter{\hobby@this@opts}%
  \ifhobby@externalise
    \ifx\hobby@path@name\pgfutil@empty
      \hobbygenusepath
    \else
      \hobbygenuseifnecpath{\hobby@path@name}%
    \fi
  \else
    \hobbygenusepath
  \fi
  \ifx\hobby@path@name\pgfutil@empty
  \else
    \hobbysavepath{\hobby@path@name}%
  \fi
  \global\let\hobby@path@name=\pgfutil@empty
  }{%
    \pgfutil@ifnextchar.{%
      \hobby@swallowdots}{%
      \tikz@scan@one@point\hobby@processpt}}}
\def\hobby@swallowdots.{%
  \pgfutil@ifnextchar.{%
    \hobby@swallowdots}{%
    \tikz@scan@one@point\hobby@processpt}}
\def\hobby@curveto@override{%
  \hobby@curveto@delegate}
\def\hobby@curveto@auto{%
  \hobbyinit\hobby@tikz@moveto\hobby@tikz@curveto\hobby@tikz@close
  \expandafter\gdef\expandafter\hobby@collected@onpath\expandafter{\expandafter{\tikz@collected@onpath}   }%
  \let\tikz@collected@onpath=\pgfutil@empty
  \pgfmathsetmacro\hobby@x{\the\tikz@lastx/1cm}%
  \pgfmathsetmacro\hobby@y{\the\tikz@lasty/1cm}%
  \xdef\hobby@initial@pt{x = \hobby@x, y = \hobby@y}%
  \expandafter\hobbysetparams\expandafter{\hobby@next@opts}%
  \expandafter\hobbyaddpoint\expandafter{\hobby@point@options,%
      x = \hobby@x, y = \hobby@y}%
  \hobby@init@tikz@commands
  \tikzset{designated Hobby path=this}%
  \let\tikz@scan@point@options=\pgfutil@empty
  \global\let\hobby@action=\pgfutil@empty
  \global\let\hobby@this@opts=\pgfutil@empty
  \global\let\hobby@next@opts=\pgfutil@empty
  \global\let\hobby@point@options=\pgfutil@empty
  \tikz@scan@one@point\hobby@addfromtikz%
}
\def\hobby@addfromtikz#1{%
  #1%
  \tikz@make@last@position{#1}%
  \pgfmathsetmacro\hobby@x{\the\pgf@x/1cm}%
  \pgfmathsetmacro\hobby@y{\the\pgf@y/1cm}%
  \expandafter\hobbysetparams\expandafter{\hobby@this@opts}%
  \expandafter\hobbyaddpoint\expandafter{\hobby@point@options,%
    x = \hobby@x, y = \hobby@y}%
  \hobby@action
  \global\let\hobby@this@opts=\pgfutil@empty
  \global\let\hobby@action=\pgfutil@empty
  \global\let\hobby@point@options=\pgfutil@empty
  \tikz@scan@next@command%
}
\def\hobby@init@tikz@commands{%
  \hobby@init@tikz@modcmd\tikz@movetoabs
  \hobby@init@tikz@modcmd\tikz@movetorel
  \hobby@init@tikz@modcmd\tikz@lineto
  \hobby@init@tikz@modcmd\tikz@rect
  \hobby@init@tikz@modcmd\tikz@cchar
  \hobby@init@tikz@modcmd\tikz@finish
  \hobby@init@tikz@modcmd\tikz@arcA
  \hobby@init@tikz@modcmd\tikz@e@char
  \hobby@init@tikz@modcmd\tikz@g@char
  \hobby@init@tikz@modcmd\tikz@schar
  \hobby@init@tikz@modcmd\tikz@vh@lineto
  \hobby@init@tikz@modcmd\tikz@pchar
  \hobby@init@tikz@modcmd\tikz@to
  \hobby@init@tikz@modcmd\pgf@stop
  \hobby@init@tikz@modcmd\tikz@decoration
  \global\let\hobby@curveto@delegate=\hobby@midcurveto@auto
}
\def\hobby@restore@tikz@commands{%
  \hobby@restore@tikz@modcmd\tikz@movetoabs
  \hobby@restore@tikz@modcmd\tikz@movetorel
  \hobby@restore@tikz@modcmd\tikz@lineto
  \hobby@restore@tikz@modcmd\tikz@rect
  \hobby@restore@tikz@modcmd\tikz@cchar
  \hobby@restore@tikz@modcmd\tikz@finish
  \hobby@restore@tikz@modcmd\tikz@arcA
  \hobby@restore@tikz@modcmd\tikz@e@char
  \hobby@restore@tikz@modcmd\tikz@g@char
  \hobby@restore@tikz@modcmd\tikz@schar
  \hobby@restore@tikz@modcmd\tikz@vh@lineto
  \hobby@restore@tikz@modcmd\tikz@pchar
  \hobby@restore@tikz@modcmd\tikz@to
  \hobby@restore@tikz@modcmd\pgf@stop
  \hobby@restore@tikz@modcmd\tikz@decoration
  \global\let\hobby@curveto@delegate=\hobby@curveto@auto
}
\def\hobby@init@tikz@modcmd#1{%
    \expandafter\global\expandafter\let\csname hobby@orig@\string#1\endcsname=#1%
    \gdef#1{\hobby@finish#1}%
}
\def\hobby@restore@tikz@modcmd#1{%
    \expandafter\global\expandafter\let\expandafter#1\csname hobby@orig@\string#1\endcsname%
}
\def\hobby@midcurveto@auto{%
  \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter\hobby@collected@onpath\expandafter\expandafter\expandafter{\expandafter\hobby@collected@onpath\expandafter{\tikz@collected@onpath}   }%
  \let\tikz@collected@onpath=\pgfutil@empty
  \let\tikz@scan@point@options=\pgfutil@empty
  \global\let\hobby@action=\pgfutil@empty
  \global\let\hobby@this@opts=\pgfutil@empty
  \global\let\hobby@point@options=\pgfutil@empty
  \tikz@scan@one@point\hobby@addfromtikz%
}
\def\hobby@finish{%
  \hobby@restore@tikz@commands
  \ifhobby@externalise
    \ifx\hobby@path@name\pgfutil@empty
      \hobbygenusepath
    \else
      \hobbygenuseifnecpath{\hobby@path@name}%
    \fi
  \else
    \hobbygenusepath
  \fi
  \ifx\hobby@path@name\pgfutil@empty
  \else
    \hobbysavepath{\hobby@path@name}%
  \fi
  \global\let\hobby@path@name=\pgfutil@empty
  \tikzset{designated Hobby path=next}%
}
\tikzset{
  quick curve through/.style={%
    to path={%
      \pgfextra{%
        \let\hobby@next@qbreak=\relax
        \let\hobby@next@qblank=\relax
      \tikz@scan@one@point\pgfutil@firstofone(\tikztostart)%
        \tikz@make@last@position{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \edef\hobby@qpoints{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \def\hobby@qpointa{}%
        \def\hobby@quick@path{}%
        \def\hobby@angle{}%
        \let\hobby@quick@curveto=\hobby@quick@makepath
        \tikz@scan@one@point\hobby@quickfirst #1 (\tikztotarget)\relax
      }
      \hobby@quick@path
    }
  },
  quick hobby/blank curve/.is choice,
  quick hobby/blank curve/true/.code={%
    \gdef\hobby@next@qblank{%
      \qhobby@blanktrue
      \global\let\hobby@next@qblank=\relax
    }%
  },
  quick hobby/blank curve/false/.code={%
    \gdef\hobby@next@qblank{%
      \qhobby@blankfalse
      \global\let\hobby@next@qblank=\relax
    }%
  },
  quick hobby/blank curve/once/.code={%
    \gdef\hobby@next@qblank{%
      \qhobby@blanktrue
      \gdef\hobby@next@qblank{%
        \qhobby@blankfalse
        \global\let\hobby@next@qblank=\relax
      }%
    }%
  },
  quick hobby/blank curve/.default=true,
  quick hobby/break curve/.is choice,
  quick hobby/break curve/true/.code={%
    \gdef\hobby@next@qbreak{%
      \qhobby@breaktrue
      \global\let\hobby@next@qbreak=\relax
    }%
  },
  quick hobby/break curve/false/.code={%
    \gdef\hobby@next@qbreak{%
      \qhobby@breakfalse
      \global\let\hobby@next@qbreak=\relax
    }%
  },
  quick hobby/break curve/once/.code={%
    \gdef\hobby@next@qbreak{%
      \qhobby@breaktrue
      \gdef\hobby@next@qbreak{%
        \qhobby@breakfalse
        \global\let\hobby@next@qbreak=\relax
      }%
    }%
  },
  quick hobby/break curve/.default=true,
}
\newif\ifqhobby@break
\newif\ifqhobby@blank
\tikzoption{hobby}[]{\let\tikz@plot@handler=\pgfplothandlerhobby}
\tikzoption{quick hobby}[]{\let\tikz@plot@handler=\pgfplothandlerquickhobby}
\tikzoption{closed hobby}[]{\let\tikz@plot@handler=\pgfplothandlerclosedhobby}
\def\hobby@quickfirst#1{%
  #1%
  \xdef\hobby@qpointa{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \tikz@make@last@position{\hobby@qpointa}%
  \pgfutil@ifnextchar\relax{%
    \xdef\hobby@quick@path{ -- (\the\pgf@x,\the\pgf@y)}%
  }{%
    \pgfutil@ifnextchar.{%
      \hobby@qswallowdots}{%
    \tikz@scan@one@point\hobby@quick}}}
\def\hobby@qswallowdots.{%
  \pgfutil@ifnextchar.{%
    \hobby@qswallowdots}{%
    \tikz@scan@one@point\hobby@quick}}
\def\hobby@quick#1{%
  \hobby@quick@compute{#1}%
  \tikz@make@last@position{\hobby@qpointa}%
  \pgfutil@ifnextchar\relax{%
    \hobby@quick@computeend%
  }{%
    \pgfutil@ifnextchar.{%
      \hobby@qswallowdots}{%
      \tikz@scan@one@point\hobby@quick}}}
\def\hobby@quick@makepath#1#2#3{%
  #1%
  \pgf@xa=\pgf@x\relax
  \pgf@ya=\pgf@y\relax
  #2%
  \pgf@xb=\pgf@x\relax
  \pgf@yb=\pgf@y\relax
  #3%
  \ifqhobby@blank
  \xdef\hobby@quick@path{\hobby@quick@path (\the\pgf@x,\the\pgf@y)}%
  \else
  \xdef\hobby@quick@path{\hobby@quick@path .. controls%
  (\the\pgf@xa,\the\pgf@ya) and (\the\pgf@xb,\the\pgf@yb) .. (\the\pgf@x,\the\pgf@y) }%
  \fi
  \ifqhobby@break
  \xdef\hobby@quick@path{\hobby@quick@path +(0,0)}%
  \fi
  \hobby@next@qbreak
  \hobby@next@qblank
}
\def\hobby@qcurveto@auto{%
  \global\let\hobby@next@qbreak=\relax
  \global\let\hobby@next@qblank=\relax
  \xdef\hobby@qpoints{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \gdef\hobby@qpointa{}%
  \gdef\hobby@quick@path{}%
  \gdef\hobby@angle{}%
  \global\let\hobby@quick@curveto=\hobby@quick@makepathauto
  \hobby@qinit@tikz@commands
  \let\tikz@scan@point@options=\pgfutil@empty
  \global\let\hobby@action=\pgfutil@empty
  \global\let\hobby@point@options=\pgfutil@empty
  \tikz@scan@one@point\hobby@qfirst@auto}
\def\hobby@qmidcurveto@auto{%
  \let\tikz@scan@point@options=\pgfutil@empty
  \global\let\hobby@action=\pgfutil@empty
  \global\let\hobby@point@options=\pgfutil@empty
  \tikz@scan@one@point\hobby@qaddfromtikz}
\def\hobby@qfirst@auto#1{%
  #1%
  \xdef\hobby@qpointa{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \tikz@make@last@position{\hobby@qpointa}%
  \tikz@scan@next@command%
}
\def\hobby@quick@makepathauto#1#2#3{%
  #1%
  \pgf@xa=\pgf@x\relax
  \pgf@ya=\pgf@y\relax
  #2%
  \pgf@xb=\pgf@x\relax
  \pgf@yb=\pgf@y\relax
  #3%
  \ifqhobby@blank
  \edef\hobby@temp{%
    \noexpand\pgfpathmoveto{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  }%
  \hobby@temp
  \else
  \edef\hobby@temp{%
    \noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  }%
  \hobby@temp
  \fi
  \ifqhobby@break
  #3%
  \edef\hobby@temp{%
    \noexpand\pgfpathmoveto{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  }%
  \hobby@temp
  \fi
  \hobby@next@qbreak
  \hobby@next@qblank
}
\def\hobby@qaddfromtikz#1{%
  \hobby@quick@compute{#1}%
  \tikz@make@last@position{\hobby@qpointa}%
  \tikz@scan@next@command%
}
\def\hobby@qinit@tikz@commands{%
  \hobby@qinit@tikz@modcmd\tikz@movetoabs
  \hobby@qinit@tikz@modcmd\tikz@movetorel
  \hobby@qinit@tikz@modcmd\tikz@lineto
  \hobby@qinit@tikz@modcmd\tikz@rect
  \hobby@qinit@tikz@modcmd\tikz@cchar
  \hobby@qinit@tikz@modcmd\tikz@finish
  \hobby@qinit@tikz@modcmd\tikz@arcA
  \hobby@qinit@tikz@modcmd\tikz@e@char
  \hobby@qinit@tikz@modcmd\tikz@g@char
  \hobby@qinit@tikz@modcmd\tikz@schar
  \hobby@qinit@tikz@modcmd\tikz@vh@lineto
  \hobby@qinit@tikz@modcmd\tikz@pchar
  \hobby@qinit@tikz@modcmd\tikz@to
  \hobby@qinit@tikz@modcmd\pgf@stop
  \hobby@qinit@tikz@modcmd\tikz@decoration
  \hobby@qinit@tikz@modcmd\tikz@@close
  \global\let\hobby@curveto@delegate=\hobby@qmidcurveto@auto
}
\def\hobby@qrestore@tikz@commands{%
  \hobby@restore@tikz@modcmd\tikz@movetoabs
  \hobby@restore@tikz@modcmd\tikz@movetorel
  \hobby@restore@tikz@modcmd\tikz@lineto
  \hobby@restore@tikz@modcmd\tikz@rect
  \hobby@restore@tikz@modcmd\tikz@cchar
  \hobby@restore@tikz@modcmd\tikz@finish
  \hobby@restore@tikz@modcmd\tikz@arcA
  \hobby@restore@tikz@modcmd\tikz@e@char
  \hobby@restore@tikz@modcmd\tikz@g@char
  \hobby@restore@tikz@modcmd\tikz@schar
  \hobby@restore@tikz@modcmd\tikz@vh@lineto
  \hobby@restore@tikz@modcmd\tikz@pchar
  \hobby@restore@tikz@modcmd\tikz@to
  \hobby@restore@tikz@modcmd\pgf@stop
  \hobby@restore@tikz@modcmd\tikz@decoration
  \hobby@restore@tikz@modcmd\tikz@@close
  \global\let\hobby@curveto@delegate=\hobby@qcurveto@auto
}
\def\hobby@qinit@tikz@modcmd#1{%
    \expandafter\global\expandafter\let\csname hobby@orig@\string#1\endcsname=#1%
    \gdef#1{\hobby@qfinish#1}%
}
\def\hobby@qfinish{%
  \hobby@quick@computeend
  \hobby@qrestore@tikz@commands
}

%% 
%% Copyright (C) 2012 by Andrew Stacey <loopspace@mathforge.org>
%% 
%% This file may be distributed and/or modified under the conditions
%% of the LaTeX Project Public License, either version 1.3 of this
%% license or (at your option) any later version.
%% The latest version of this license is in:
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%% 
%% This work is "maintained" (as per LPPL maintenance status) by
%% Andrew Stacey.
%% 
%% This work consists of the files  hobby.dtx
%%                                  hobby_doc.tex
%% and the derived files            hobby.code.tex
%%                                  pgflibraryhobby.code.tex
%%                                  tikzlibraryhobby.code.tex
%%                                  pml3array.sty
%%                                  hobby.ins
%%                                  hobby.pdf
%%                                  hobby_code.pdf
%%                                  README.txt
%% 
%%
%% End of file `tikzlibraryhobby.code.tex'.

